Deep Ensembles for Low-Data Transfer Learning

In the low-data regime, it is difficult to train good supervised models from scratch. Instead practitioners turn to pre-trained models, leveraging transfer learning. Ensembling is an empirically and theoretically appealing way to construct powerful predictive models, but the predominant approach of training multiple deep networks with different random initialisations collides with the need for transfer via pre-trained weights. In this work, we study different ways of creating ensembles from pre-trained models. We show that the nature of pre-training itself is a performant source of diversity, and propose a practical algorithm that efficiently identifies a subset of pre-trained models for any downstream dataset. The approach is simple: Use nearest-neighbour accuracy to rank pre-trained models, fine-tune the best ones with a small hyperparameter sweep, and greedily construct an ensemble to minimise validation cross-entropy. When evaluated together with strong baselines on 19 different downstream tasks (the Visual Task Adaptation Benchmark), this achieves state-of-the-art performance at a much lower inference budget, even when selecting from over 2,000 pre-trained models. We also assess our ensembles on ImageNet variants and show improved robustness to distribution shift.

==> sections/results_old.tex <==
\clearpage

\section{OLD RESULTS SECTION}
\subsection{Expert ensembles vs. baselines}

\CRR{Personally, I'd avoid using BiT-L and BiT-M too much. I think it's confusing as it requires the reader to know previous papers. I mean, it's fine to put that in tables, but if we can say R50 trained on Imagenet21k or JFT instead, I think it's simpler to digest...}
\JP{Using BiT-L and BiT-M can save a lot of space in the text.}

We first consider ResNet-50s trained on JFT - both BiT-L (trained on the entire dataset) and expert models trained on subsets \JP{This is in line two what is shown in \citep{puigcerver2020experts}}. For simplicity, here we report test performances; it is clear that ExpertEnsembles outperform both HyperEnsembles and AugEnsembles at all ensemble sizes.\\
More thorough analysis on validation data is available in Appendix \ref{app:baselines}. In particular, we explore the role of the $k$NN in the ExpertEnsembles. We find that random selection of pre-trained feature extractors performs notably worse; diversity in initialisation simply for the sake of diversity is by itself not sufficient.
\CRR{If you think about it, this is quite remarkable. The random experts are finetuned on the downstream data, still they do so poorly... I imagine their representations are crap for the task at hand? So crap that even after finetuning+ensembling they can't recover... 5 points difference on average with experts...}
In fact, we found that when not using the $k$NN at all and training \textit{all} available JFT R50 experts, performance dropped slightly - we suspect this is because, when passed 976 models to choose from, the greedy algorithm overfits (see Appendix \ref{app:knn}).
\CRR{This is also remarkable iiuc. No matter how many models you throw at kNN, it'll do the approx right thing.}
Further discussion on the contribution of the $k$NN, and the greedy variant we tried, is in Appendix \ref{app:knn}.\\
We experiment similarly with feature extractors pre-trained on ImageNet21k and show a similar trend - hyper ensembles are performant, but expert ensembles from pretraining specialisation give a further performance boost.

% \subsection{The ensemble selection and construction process}
% \subsubsection{Variants to KNN selection}
% In the base algorithm, the candidate feature extractors are the top $K$ according to KNN accuracy. Similar to the greedy ensemble construction algorithm, we consider a greedy approach to selecting feature extractors in KNN space, with the goal of selecting feature extractors that we expect would ensemble well together after finetuning on the target dataset. To do this, we consider the classification picked by the KNN leave-one-out classifier as a (one-hot) probability distribution. KNN ensembles are constructed by averaging these classifications; we greedily choose feature extractors so as to minimise cross-entropy.\\
% Figure \ref{fig:knn_selection} shows the effect of using this greedy method with the JFT R50 and R50 INet21k expert ensembles. There are no clear gains from this approach.
% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{images/knn_vs_greedy.png}
%     \caption{ExpertEnsembles selected with different KNN approaches.}
%     \label{fig:knn_selection}
% \end{figure}

\subsubsection{Combining approaches}
As discussed in Section \ref{sec:combine}, we can combine expert ensembles with hyper/augmentation ensembles. More details on this are in Appendix \ref{app:combine}, but we see that, the simple thresholding by KNN accuracy approach works well, giving a small boost in test performance (Table \ref{tab:test}). Our highest performing ResNet50 ensembles combine the ExpertEnsemble with the AugEnsembles.

% \begin{wrapfigure}[11]{r}{0.46\textwidth}
% % \vspace{-1cm}
%     \centering
%     \includegraphics[width=0.45\textwidth]{images/finetuning_budget_single.png}
%     \caption{Effect of the finetuning budget on ensemble performance.}
%     \label{fig:finetuning_budget_ensemble_size}
% \end{wrapfigure}
% \subsubsection{Effect of finetuning budget}
% In the previous experiments, and the majority of coming experiments, we allow the KNN to pick $N = 15$ experts. Stacking the default four hyperparameters yields a finetuning budget of 60 models - i.e. this is the number of models trained for a given task (and the majority of compute expenditure incurred by a practitioner, as the KNN selection and ensembling are comparitively cheap). The hyperensemble was run with the same fine-tuning budget budget (max 60 models).\\
% Figure \ref{fig:finetuning_budget_ensemble_size} shows how performance drops as a function of this fine-tuning budget. Interestingly, the expert ensembles are actually more robust to this fine-tuning budget, retaining higher performance when training less models, indicating the $k$NN's usefulness as a pre-selection phase.

\subsubsection{Model scale}
One form of diversity that can still be exploited for transfer learning is diversity in the architecture of pretrained models. We consider 18, 34, 50 and 101 layer ResNets trained on JFT subsets, starting from generalist models. This is explored more thoroughly in Appendix \ref{app:scale}. In particular, when selecting from ResNet-18s, 34s and 50s pre-trained on JFT, we get a further performance boost. Though one might expect the KNN selection and/or greedy algorithm to be biased towards selecting larger architectures, the final ensembles contain a mix of architecture scales, with some datasets seeing increased performance as a result of this mix.\\
% \BM{Interesting notes (not sure what to include)}
% \begin{itemize}
%     \item Larger architecture isn't always best - e.g. for dsprites.xpos, when picking only R18s, it gets an 8\% improvement over the R101 ensemble
%     \item Gains to some extent stack with architecture size
%     \item Both KNN and greedy algorithm pick a diverse set of architectures.
%     \item To some extent, diversity in architecture + pretraining data may be marginally more useful than diversity in pretraining data alone (from dedup)
%     \item We get a minor boost from selecting from JFT R18s/R34s/R50s vs. just selecting R50s
% \end{itemize}

\noindent
\begin{minipage}{.55\textwidth}
\subsubsection{Effect of finetuning budget}
In the previous experiments, and the majority of coming experiments, we allow the $k$NN to pick $N = 15$ experts. Stacking the default four hyperparameters yields a finetuning budget of 60 models - i.e. this is the number of models trained for a given task (and the majority of compute expenditure incurred by a practitioner, as the $k$NN selection and ensembling are comparitively cheap). The hyperensemble was run with the same fine-tuning budget (max 60 models). Figure \ref{fig:finetuning_budget_ensemble_size} shows how performance drops with reduced fine-tuning budget. Interestingly, the expert ensembles are actually more robust to this, retaining higher performance when training less models, indicating the $k$NN's usefulness as a pre-selection phase.
\end{minipage}\hspace{0.2cm}
\begin{minipage}{.43\textwidth}
% \begin{figure}
\centering
\includegraphics[width=0.98\textwidth]{images/finetuning_budget_single.png}
\captionof{figure}{Effect of the finetuning budget on ensemble performance.}
\label{fig:finetuning_budget_ensemble_size}
% \end{figure}
\end{minipage}

\subsection{Final VTAB performance}
We assess the hyperensembles, and some of the expert ensembles, on VTAB-1K. Performances are shown in Table \ref{tab:test}. The expert ensembles outperform hyperensembles, in particular experiencing large gains on natural tasks.\\
We also show BiT models from \citep{alex2019big}, which until now have been the highest performers on VTAB-1K. Firstly, it is clear from comparing to the single fine-tuned generalist ResNet-50s that both HyperEnsembles and ExpertEnsembles dramatically improve performance over a single model, as one would expect.  Notably however, even our ResNet-50 ExpertEnsemble and hybrid ensembles outperform the leading model, a much larger BiT-L ResNet152x4.\\
Secondly, one can see that there is some merit to the hybrid approach for both JFT and ImageNet21k. We can also see from the ResNet-101 results that the gains from ensembling stack with scale.\\
Finally, the `All Experts' entry is particularly interesting; the KNN had to select $K = 15$ feature extractors from a pool of 2002 candidates (all the experts described in Appendix \ref{app:training_fes}). Overall, it achieved comparable performance to just picking from the pool of ResNet-101s. % Better spin required here!
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht]
\centering
\begin{tabular}{@{}lcGGG@{}}
\toprule
Description           & VTAB-1K  & Natural & Specialised & Structured \\ \midrule
JFT R50 Experts           & 76.4\rng{76.1}{76.6} & 82.2   & 85.6       & 66.8      \\
JFT R18/34/50 Experts     & 76.8\rng{76.4}{77.2} & 82.2  &  85.5       & 67.9  \\
BiT-L R50 Hypers          & 75.6\rng{75.2}{75.7} & 80.1   & 85.6       & 66.6      \\
BiT-L R50 Augs            & 73.1\rng{72.8}{73.3} & 80.6   & 86.9       & 59.6      \\
JFT R50 HyperExperts      & 76.6\rng{76.0}{76.7} & 82.5   & 85.8       & 66.8      \\
JFT R50 AugExperts        & 76.8\rng{76.6}{76.9} & 82.6   & 86.0       & 67.2      \\
\midrule
INet21k R50 Experts       & 75.3\rng{74.5}{75.6} & 79.9   & 85.7        & 66.1      \\
BiT-M R50 Hypers          & 74.2\rng{73.7}{74.8} & 79.6   & 86.2        & 63.5      \\
INet21k R50 HyperExperts  & 75.6\rng{74.8}{75.8} & 79.9   & 85.5        & 67.0      \\ \midrule
% JFT + INet21k Experts & 76.34 & 81.71   & 86.08        & 66.76      \\ \midrule
JFT R101 experts      & \textbf{77.6}\rng{77.4}{77.8} & 83.6   & 86.4        & 68.0      \\
All Experts           & 77.6\rng{77.3}{77.7} & 83.6   & 86.1        & 68.1      \\ \midrule
BiT-L R50$^*$           & 70.6\phantom{\rng{77.7}{77.7}} & 77.8   & 83.6        & 57.9      \\
BiT-M R50$^*$           & 70.0\phantom{\rng{77.7}{77.7}} & 77.0   & 84.7        & 56.6      \\
BiT-L R152x4$^*$          & 76.2\phantom{\rng{77.7}{77.7}} & 86.0   & 87.0       & 62.2      \\ \bottomrule
\end{tabular}
\caption{Test accuracies of different ensembles and baselines from \citet{zhai2019largescale} [$^*$].
%\DK{personal opinion: I think using only one significant digit after the decimal is better to read and also more reasonable seeing the ranges - saw that this was started and finished this now, rounding based on the two significant digits that were here. This could have lead to double-rounding errors, e.g. 85.5476 -> 85.55 -> 85.6, so would need to go back to the original numbers for a final pass, if you tell me where the numbers are.} 
\CRR{Original Table -- kept for reference after splitting.}
}

\label{tab:test}
\end{table}

\subsection{Inference cost}
We limited the number of models in the final ensemble to 15, regardless of whether the greedy algorithm indicated more may be better. For single models, it was generally found that larger models perform stronger across an array of downstream tasks \citep{alex2019big}; overall however, expert ensembles outperform these larger models on average across diverse tasks. \AP{Should be more "pessimistic" and clearly point out that it only works out very well in structured and that is enough to bring the average performance match the BiT-L R152x4?}\\
Figure \ref{fig:flops} shows a comparison of the inference FLOPs of different leading models on VTAB vs the ensembles developed here. Both the hyperensembles and the expert ensembles perform favourably, giving higher performance with a lower inference cost on average when compared to large finetuned generalist models from \citep{alex2019big}.

\subsection{Robustness to Distribution Shift}
Previous work has shown ensembles perform well when considering metrics relating to uncertainty and out of distribution detection \citep{balaji2017ensembles,stickl2020diverse}.

% \subsubsection{Something about analysing the experts}
% \BM{IN PROGRESS! We haven't figured out the best way to analyse this yet}
% For both the HyperEnsembles and the ExpertEnsembles, we analyse the predictions of each ensemble member on the test data of \textit{all} VTAB datasets, including the ones it was not trained on. Though there are many measures of ensemble diversity \citep{kuncheva2003diversity}, we look at the entropy of predictions - other metrics, such as cosine distance, revealed the same trends discussed below. Similar to previous studies, we find that our more accurate expert ensembles also have higher diversity/disagreement on \textbf{in-distribution} test data.


% As well as high accuracy on the distribution it was trained on, we aim for regularised ensembles which aren't overconfident; for example, they should have higher disagreement on out of distribution data \citep{balaji2017ensembles}. Figure \ref{fig:diversity_ood} shows the distribution of prediction entropy across VTAB; the expert ensembles are indeed also superior on this front.

% \CRR{Current plots point in the right direction but aren't super conclusive. I'd probably split by dataset the VTAB one. Not sure entropy is the most intuitive metric to share.}

% \begin{figure}
% \centering
% \begin{subfigure}{.4\textwidth}
%   \centering
%   \includegraphics[width=.98\linewidth]{images/test_id_disagreement_entropy.png}
%   \caption{In distribution VTAB predictions}
%   \label{fig:diversity_id}
% \end{subfigure}%
% \begin{subfigure}{.4\textwidth}
%   \centering
%   \includegraphics[width=.98\linewidth]{images/test_ood_disagreement_entropy.png}
%   \caption{Out of distribution VTAB predictions}
%   \label{fig:diversity_ood}
% \end{subfigure}
% \caption{Model diversity as measured by entropy on in-distribution and out-of-distribution data in VTAB.
% \CRR{I'd rethink these plots a bit. Let's chat offline.}}
% \label{fig:diversity}
% \end{figure}



% \subsubsection{ImageNet Robustness Metrics}
We first create HyperEnsembles and ExpertEnsembles for the ImageNet classification task. For the former, we create a hyperensemble as described before using the BiT-L R50x1 as the base feature extractor. For the latter, we use the JFT R50x1 experts, using 50,000 examples from the training set to run the KNN algorithm to pick feature extractors before training. For both, we use the entire validation set to inform ensembling decisions.

Note that we are no longer in the low data regime, where we expect the benefits of this approach to be most evident.
Once the ensembles are trained and constructed, we assess them on a suite of datasets aiming to quantify robustness to distribution shift. More information is included in Appendix \ref{app:imagenet}, but each dataset introduces some form of distribution shift; some are artificial (ImageNet C), others are due to data recollection (ImageNet A/R/v2, ObjectNet) and the remaining are due to natural invariances in video (YTBB, ImageNet Vid). Figure \ref{fig:robustness} shows these metrics; As well as having a slightly better accuracy on the held out data, the expert ensembles perform significantly better under distribution shift.

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{images/robustness.png}
%     \caption{Robustness and uncertainty metrics hyperensembles vs. expert ensembles}
%     \label{fig:robustness}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{images/robustness_accs.png}
    \caption{\textbf{Expert ensembles retain higher accuracy under domain shift}. Aside from the first row, which shows test accuracy, all other rows correspond to some kind of induced distribution shift, either artificially or otherwise. In all bar one, we get significant boosts in accuracy compared to the HyperEnsembles. Note that we have inverted some rows such that higher is always better e.g. \textit{lower} accuracy drop is better for video metrics, but we plot the negative of that for easy interpretation.}
    \label{fig:robustness}
\end{figure}

==> tables/domain_adaptive_transfer.tex <==
% See main.tex to understand what \civ{}{}{} does.
\setlength{\tabcolsep}{2pt}
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{llllllll}
\toprule
%    & Aircraft & Birds & Cars & \hspace{-1ex}CIFAR10 & Food & Pets & Avg.\\
& \textsc{Aircraft} & \textsc{Birds} & \textsc{Cars} & \textsc{CIFAR10} & \textsc{Food} & \textsc{Pets}* & \textsc{Avg.}\\    
\midrule  
% \cit{Baseline (R50)}
%   & \civ{91.4}{91.0}{91.7} & \civ{78.8}{78.0}{79.4} & \civ{95.6}{95.4}{95.7} & \civ{97.8}{97.7}{97.9} & \civ{91.3}{91.2}{91.5} & \civ{94.6}{94.5}{94.7} & \civ{91.6}{91.4}{91.7} \\
% \cit{Adapter Experts}
%   & \civ{92.5}{92.2}{92.8} & \civ{79.4}{78.7}{80.1} & \civ{95.9}{95.8}{96.0} & \civ{97.9}{97.8}{98.0} & \civ{91.6}{91.5}{91.7} & \civ{94.7}{94.5}{94.9} & \civ{92.0}{91.9}{92.1} \\
% \cit{Full Experts}
%   & \civ{\textbf{94.8}}{94.5}{95.1} & \civ{\textbf{83.6}}{83.1}{83.9} & 
%   \civ{\textbf{96.1}}{96.0}{96.3} & \civ{97.8}{97.7}{97.9} & 
%   \civ{93.1}{92.8}{93.2} & \civ{\textbf{97.0}}{96.9}{97.1} & 
%   \civ{\textbf{93.7}}{93.6}{93.8} \\
Baseline
  & \cih{91.4}{91.0}{91.7} & \cih{78.8}{78.0}{79.4} & \cih{95.6}{95.4}{95.7} & \cih{97.8}{97.7}{97.9} & \cih{91.3}{91.2}{91.5} & \cih{94.5}{94.4}{94.6} & \cih{91.6}{91.4}{91.7} \\
Adapters (JFT)
  & \cih{92.5}{92.2}{92.8} & \cih{79.4}{78.7}{80.1} & \cih{95.9}{95.8}{96.0} & \cih{97.9}{97.8}{98.0} & \cih{91.6}{91.5}{91.7} & \cih{94.6}{94.4}{94.8} & \cih{92.0}{91.9}{92.1} \\
Full (JFT)
  & \cih{\textbf{94.8}}{94.5}{95.1} & \cih{{83.6}}{83.1}{83.9} & 
  \cih{\textbf{96.1}}{96.0}{96.3} & \cih{97.8}{97.7}{97.9} & 
  \cih{93.1}{92.8}{93.2} & \cih{\textbf{97.0}}{96.9}{97.1} & 
  \cih{93.7}{93.6}{93.8} \\
\midrule
%%%%%%%%%%%%%% DAT paper
% Baseline (Iv3) \cite{ngiam2018domain}
%   & 88.2& 74.2& 94.0& 97.6& 88.6& 92.5& 89.2\\
Dom-Ad (In-v3) \cite{ngiam2018domain}
  & 94.1 & 81.7 & 95.7 & {98.3} & {94.1} & \textbf{97.1} & 93.5 \\ 
Dom-Ad (Am-B) \cite{ngiam2018domain}
  & 92.8 & \textbf{85.1} & 95.8 & \textbf{98.6} & \textbf{95.3} & {96.8} & \textbf{94.1} \\ 
\bottomrule
\end{tabular}
}
\begin{flushleft}
\small{*Pets results are mean per class accuracy as opposed to mean accuracy.}\end{flushleft}\vspace{-0.5cm}

==> tables/domain_adaptive_transfer_details.tex <==
% See main.tex to understand what \civ{}{}{} does.
\setlength{\tabcolsep}{2pt}
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{llllllll}
\toprule
    & Aircraft & Birds & Cars & \hspace{-1ex}CIFAR10 & Food & Pets* & Avg.\\
\midrule
%%%%%%%%%%%%%% KNN
Baseline
& \cih{91.4}{91.0}{91.7} 
& \cih{78.8}{78.0}{79.4} 
& \cih{95.6}{95.4}{95.7} 
& \cih{97.8}{97.7}{97.9} 
& \cih{91.3}{91.2}{91.5} 
& \cih{94.5}{94.4}{94.6} 
& \cih{91.6}{91.4}{91.7} \\
kNN & & & & & & &\\
~~Adapters, 4e
& \cih{92.5}{92.2}{92.8} 
& \cih{79.4}{78.7}{80.1} 
& \cih{95.9}{95.8}{96.0} 
& \cih{97.9}{97.8}{98.0} 
& \cih{91.6}{91.5}{91.7} 
& \cih{94.6}{94.4}{94.8} 
& \cih{92.0}{91.9}{92.1} \\
~~Full, 2e
& \cih{94.5}{94.2}{94.7} 
& \cih{83.5}{83.1}{83.9} 
& \cih{96.0}{95.8}{96.2} 
& \cih{97.9}{97.8}{98.0} 
& \cih{92.9}{92.8}{93.1} 
& \cih{96.8}{96.7}{96.9} 
& \cih{93.6}{93.5}{93.7} \\
~~Full, 4e
& \cih{\textbf{94.8}}{94.5}{95.1} 
& \cih{83.6}{83.1}{83.9} 
& \cih{96.1}{96.0}{96.3} 
& \cih{97.8}{97.7}{97.9} 
& \cih{93.1}{92.8}{93.2} 
& \cih{\textbf{97.0}}{96.9}{97.1} 
& \cih{93.7}{93.6}{93.8} \\
%%%%%%%%%%%%%% KL
KL & & & & & & &\\
~~Adapters, 4e
& \cih{92.1}{91.8}{92.5} 
& \cih{80.0}{79.5}{80.4} 
& \cih{95.9}{95.8}{96.0} 
& \cih{97.9}{97.8}{98.0} 
& \cih{91.6}{91.5}{91.8} 
& \cih{94.5}{94.3}{94.7} 
& \cih{92.0}{91.9}{92.1} \\
~~Full, 2e
& \cih{94.6}{93.6}{95.0} 
& \cih{83.1}{82.6}{83.5} 
& \cih{96.1}{96.0}{96.2}
& \cih{97.9}{97.8}{98.1} 
& \cih{92.9}{92.9}{93.1} 
& \cih{96.6}{96.5}{96.7} 
& \cih{93.5}{93.4}{93.7} \\
~~Full, 4e
& \cih{94.4}{94.1}{94.7} 
& \cih{83.7}{83.3}{84.3} 
& \cih{\textbf{96.4}}{96.3}{96.4} 
& \cih{97.9}{97.8}{98.0} 
& \cih{93.1}{92.9}{93.3} 
& \cih{96.6}{96.6}{96.6} 
& \cih{93.7}{93.6}{93.8} \\
%%%%%%%%%%%%%% EPN
EPN & & & & & & &\\  
~~Adapters, 4e
& \cih{92.1}{91.7}{92.5} 
& \cih{79.7}{79.1}{80.2} 
& \cih{95.8}{95.6}{96.0} 
& \cih{97.3}{97.1}{97.4} 
& \cih{91.5}{91.3}{91.7} 
& \cih{93.1}{91.8}{93.6} 
& \cih{91.6}{91.4}{91.8} \\
~~Full, 2e
& \cih{94.0}{93.6}{94.3} 
& \cih{83.3}{82.7}{83.9}
& \cih{96.2}{96.1}{96.2} 
& \cih{96.9}{96.7}{97.1} 
& \cih{92.5}{92.3}{92.6} 
& \cih{\textbf{97.0}}{97.0}{97.1} 
& \cih{93.3}{93.2}{93.4} \\
~~Full, 4e
& \cih{94.2}{94.1}{94.4}
& \cih{84.3}{83.9}{84.7} 
& \cih{96.0}{96.0}{96.1} 
& \cih{96.6}{96.4}{96.7} 
& \cih{92.4}{92.3}{92.6} 
& \cih{96.9}{96.9}{97.0} 
& \cih{93.4}{93.3}{93.5} \\
\midrule
Dom-Ad (In-v3) \cite{ngiam2018domain}
  & 94.1 & 81.7 & 95.7 & {98.3} & {94.1} & \textbf{97.1} & 93.5 \\ 
Dom-Ad (Am-B) \cite{ngiam2018domain}
  & 92.8 & \textbf{85.1} & 95.8 & \textbf{98.6} & \textbf{95.3} & {96.8} & \textbf{94.1} \\ 
\bottomrule
\end{tabular}
}
\begin{flushleft}
\small{*Pets results are mean per class accuracy as opposed to mean accuracy.}\end{flushleft}\vspace{-0.5cm}

==> tables/selection_algorithms.tex <==
\begin{tabular}{lllll}
\toprule
& \textsc{Natural} & \textsc{Specialized} & \textsc{Structured} & \textsc{All}\\
\midrule
%% Full experts.
Random
& \cih{60.6}{59.1}{63.9} 
& \cih{81.2}{80.9}{81.8} 
& \cih{56.8}{54.9}{57.8} 
& \cih{63.3}{62.3}{64.6} \\
Domain Prediction
& \cih{75.9}{74.4}{77.4} 
& \cih{81.5}{81.3}{82.2} 
& \cih{\textbf{57.0}}{56.1}{57.4} 
& \cih{69.1}{68.4}{69.8} \\
Label Matching
& \cih{77.6}{77.8}{78.1} 
& \cih{80.3}{79.1}{82.5}
& \cih{56.9}{55.6}{57.2} 
& \cih{69.6}{68.9}{70.0} \\
Performance Proxy
& \cih{\textbf{79.7}}{79.5}{80.0} 
& \cih{\textbf{83.6}}{83.3}{83.8} 
& \cih{55.3}{52.1}{56.3} 
& \cih{\textbf{70.2}}{68.9}{70.6}\\
% Random
% & \cih{60.64}{59.05}{63.89} 
% & \cih{81.22}{80.90}{81.75} 
% & \cih{56.77}{54.85}{57.84} 
% & \cih{63.34}{62.34}{64.60} \\
% Domain Prediction
% & \cih{75.88}{74.35}{77.36} 
% & \cih{81.49}{81.32}{82.24} 
% & \cih{\textbf{57.00}}{56.14}{57.44} 
% & \cih{69.11}{68.35}{69.78} \\
% Label Matching
% & \cih{77.95}{77.82}{78.14} 
% & \cih{80.32}{79.10}{82.48}
% & \cih{56.92}{55.60}{57.19} 
% & \cih{69.59}{68.93}{70.02} \\
% Performance Proxy
% & \cih{\textbf{79.65}}{79.51}{79.96} 
% & \cih{\textbf{83.55}}{83.25}{83.80} 
% & \cih{55.26}{52.11}{56.25} 
% & \cih{\textbf{70.20}}{68.89}{70.62}\\
%% Adapters experts.  
% Random
%   & \cih{58.60}{56.08}{59.64} & \cih{78.25}{76.75}{79.17} & \cih{58.64}{57.83}{59.60} & \cih{62.75}{61.71}{63.32} \\
% Domain Prediction
%   & \cih{70.79}{69.29}{71.57} & \cih{75.49}{63.69}{77.96} & \cih{59.70}{58.24}{60.95} & \cih{67.11}{64.50}{67.93} \\
% Label Matching
%   & \cih{75.32}{75.13}{75.40} & \cih{80.48}{78.16}{81.25} & \cih{56.06}{51.82}{56.99} & \cih{68.30}{66.40}{68.70} \\
% Performance Proxy
%   & \cih{78.96}{78.60}{79.07} & \cih{81.34}{79.21}{82.48} & \cih{59.07}{58.28}{60.07} & \cih{71.09}{70.54}{71.57} \\
\bottomrule     
\end{tabular}

==> tables/selection_algorithms_detailed.tex <==
\begin{tabular}{lllll}
\toprule
& \textsc{Natural} & \textsc{Specialized} & \textsc{Structured} & \textsc{All}\\
\midrule  
\emph{Adapters} & & & &\\
~~Random
  & \cih{58.6}{56.1}{59.6} 
  & \cih{78.3}{76.8}{79.2} 
  & \cih{58.6}{57.8}{59.6} 
  & \cih{62.8}{61.7}{63.3} \\
~~Domain Prediction
  & \cih{70.8}{69.3}{71.6} 
  & \cih{75.5}{63.7}{78.0} 
  & \cih{59.7}{58.2}{61.0} 
  & \cih{67.1}{64.5}{67.9} \\
~~Label Matching
  & \cih{75.3}{75.1}{75.4} 
  & \cih{80.5}{78.2}{81.3} 
  & \cih{56.1}{51.8}{57.0} 
  & \cih{68.3}{66.4}{68.7} \\
~~Performance Proxy
  & \cih{79.0}{78.6}{79.1} 
  & \cih{81.3}{79.2}{82.5} 
  & \cih{59.1}{58.3}{60.1} 
  & \cih{71.1}{70.5}{71.6} \\
\midrule
\emph{Full} & & & &\\
~~Random
  & \cih{60.6}{59.1}{63.9} 
  & \cih{81.22}{80.9}{81.8} 
  & \cih{56.8}{54.9}{57.8} 
  & \cih{63.3}{62.3}{64.6} \\
~~Domain Prediction
  & \cih{75.9}{74.4}{77.4} 
  & \cih{81.5}{81.3}{82.2} 
  & \cih{\textbf{57.0}}{56.1}{57.4} 
  & \cih{69.1}{68.4}{69.8} \\
~~Label Matching
  & \cih{78.0}{77.8}{78.1} 
  & \cih{80.3}{79.1}{82.5} 
  & \cih{56.9}{55.6}{57.2} 
  & \cih{69.6}{68.9}{70.0} \\
~~Performance Proxy
  & \cih{\textbf{79.7}}{79.5}{80.0} 
  & \cih{\textbf{83.6}}{83.3}{83.8} 
  & \cih{55.3}{52.1}{56.3} 
  & \cih{\textbf{70.2}}{68.9}{70.6} \\
\bottomrule     
\end{tabular}

==> tables/vtab_detailed.tex <==
{\setlength{\tabcolsep}{2pt}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrr}
\toprule
& \rotatebox[origin=l]{90}{\naturalsym~caltech101}
& \rotatebox[origin=l]{90}{\naturalsym~cifar100}
& \rotatebox[origin=l]{90}{\naturalsym~dtd}
& \rotatebox[origin=l]{90}{\naturalsym~flowers}
& \rotatebox[origin=l]{90}{\naturalsym~pets}
& \rotatebox[origin=l]{90}{\naturalsym~sun397}
& \rotatebox[origin=l]{90}{\naturalsym~svhn}
& \rotatebox[origin=l]{90}{\specializedsym~camelyon}
& \rotatebox[origin=l]{90}{\specializedsym~eurosat}
& \rotatebox[origin=l]{90}{\specializedsym~retino}
& \rotatebox[origin=l]{90}{\specializedsym~resisc45}
& \rotatebox[origin=l]{90}{\structuredsym~clevr.closest}
& \rotatebox[origin=l]{90}{\structuredsym~clevr.count}
& \rotatebox[origin=l]{90}{\structuredsym~dmlab}
& \rotatebox[origin=l]{90}{\structuredsym~dsprites.orient}
& \rotatebox[origin=l]{90}{\structuredsym~dsprites.xpos}
& \rotatebox[origin=l]{90}{\structuredsym~kitti}
& \rotatebox[origin=l]{90}{\structuredsym~smallnorb.azmth}
& \rotatebox[origin=l]{90}{\structuredsym~smallnorb.elev}
\\
\midrule
\emph{JFT} & & & & & & & & & & & & & & & & & & & \\
\cit{~~Baseline}
& \civ{91.7}{91.5}{91.8} 
& \civ{68.6}{68.3}{68.7} 
& \civ{72.1}{72.0}{72.2} 
& \civ{97.2}{97.1}{97.2} 
& \civ{91.5}{91.4}{91.5} 
& \civ{49.9}{49.9}{50.0} 
& \civ{71.2}{70.5}{72.0} 
& \civ{81.6}{81.4}{83.1} 
& \civ{93.0}{92.9}{93.1} 
& \civ{70.0}{69.6}{70.2} 
& \civ{81.8}{81.5}{81.9} 
& \civ{54.9}{54.5}{55.8} 
& \civ{62.8}{60.7}{68.0} 
& \civ{45.1}{45.0}{45.3} 
& \civ{61.6}{61.1}{62.1} 
& \civ{94.9}{93.7}{96.2} 
& \civ{79.8}{43.9}{80.8} 
& \civ{25.1}{22.0}{30.5} 
& \civ{33.6}{33.1}{35.5} 
\\
\cit{~~Adapters (EPN)}
& \civ{91.7}{91.6}{91.7} 
& \civ{34.0}{32.2}{34.3} 
& \civ{58.3}{58.0}{58.6} 
& \civ{98.2}{98.1}{98.2} 
& \civ{91.4}{91.3}{91.5} 
& \civ{48.3}{48.1}{48.4} 
& \civ{73.7}{63.3}{79.2} 
& \civ{79.6}{71.7}{83.1} 
& \civ{93.1}{92.2}{93.6} 
& \civ{60.0}{53.7}{66.4} 
& \civ{69.3}{23.3}{74.3} 
& \civ{60.6}{57.3}{61.9} 
& \civ{63.3}{56.7}{73.3} 
& \civ{45.1}{43.7}{46.0} 
& \civ{59.3}{56.9}{59.5} 
& \civ{95.8}{95.0}{96.8} 
& \civ{79.2}{73.7}{80.4} 
& \civ{32.6}{32.1}{33.1} 
& \civ{41.8}{37.7}{42.6} 
\\
\cit{~~Adapters (KL)}
& \civ{91.4}{91.1}{91.6} 
& \civ{68.3}{68.2}{68.3} 
& \civ{57.5}{57.0}{57.7} 
& \civ{98.1}{97.8}{98.2} 
& \civ{92.0}{91.9}{92.0} 
& \civ{48.3}{48.3}{48.4} 
& \civ{71.6}{70.9}{72.1} 
& \civ{83.0}{74.1}{83.6} 
& \civ{93.0}{92.9}{93.1} 
& \civ{68.2}{64.5}{70.7} 
& \civ{77.7}{77.5}{79.7} 
& \civ{52.2}{49.3}{53.8} 
& \civ{59.9}{58.3}{62.3} 
& \civ{43.8}{41.7}{45.0} 
& \civ{61.2}{59.9}{62.1} 
& \civ{94.1}{90.8}{96.1} 
& \civ{77.9}{47.0}{79.0} 
& \civ{24.9}{16.8}{30.4} 
& \civ{34.4}{33.4}{35.4} 
\\
\cit{~~Adapters (kNN)}
& \civ{91.6}{91.5}{91.7} 
& \civ{68.4}{68.3}{68.6} 
& \civ{72.2}{72.1}{72.2} 
& \civ{97.7}{97.7}{97.8} 
& \civ{91.9}{91.8}{92.0} 
& \civ{49.8}{49.8}{49.9} 
& \civ{81.1}{78.7}{81.8} 
& \civ{83.3}{82.8}{83.7} 
& \civ{93.0}{93.0}{93.1} 
& \civ{67.3}{58.8}{71.8} 
& \civ{81.7}{81.5}{81.8} 
& \civ{61.2}{59.1}{62.1} 
& \civ{78.0}{75.0}{79.5} 
& \civ{44.9}{44.3}{46.2} 
& \civ{61.8}{61.3}{62.2} 
& \civ{89.3}{87.5}{92.8} 
& \civ{78.8}{77.6}{79.4} 
& \civ{24.1}{23.7}{26.6} 
& \civ{34.5}{30.3}{40.7} 
\\
\cit{~~Full (EPN)}
& \civ{91.6}{91.2}{91.7} 
& \civ{53.2}{53.1}{53.4} 
& \civ{63.3}{63.0}{63.6} 
& \civ{99.5}{99.5}{99.5} 
& \civ{96.1}{96.1}{96.2} 
& \civ{55.1}{55.0}{55.1} 
& \civ{72.3}{61.7}{82.6} 
& \civ{83.3}{82.9}{84.1} 
& \civ{94.0}{93.9}{94.1} 
& \civ{74.1}{73.9}{74.2} 
& \civ{74.5}{74.3}{77.1} 
& \civ{56.8}{55.2}{57.9} 
& \civ{62.9}{60.6}{65.5} 
& \civ{38.2}{37.4}{39.5} 
& \civ{64.2}{63.1}{64.5} 
& \civ{96.5}{95.5}{97.0} 
& \civ{75.5}{74.4}{76.1} 
& \civ{22.8}{19.1}{23.3} 
& \civ{39.1}{38.7}{39.7} 
\\
\cit{~~Full (KL)}
& \civ{91.6}{91.5}{91.7} 
& \civ{68.4}{68.2}{68.6} 
& \civ{64.3}{63.8}{64.7} 
& \civ{99.5}{99.5}{99.5} 
& \civ{95.9}{95.9}{95.9} 
& \civ{55.1}{55.1}{55.2} 
& \civ{70.7}{70.2}{71.8} 
& \civ{83.1}{81.8}{83.5} 
& \civ{93.0}{92.9}{93.0} 
& \civ{61.8}{57.4}{70.4} 
& \civ{83.4}{83.4}{83.5} 
& \civ{54.0}{50.3}{55.3} 
& \civ{60.6}{56.5}{61.3} 
& \civ{45.1}{41.5}{45.2} 
& \civ{64.5}{62.9}{65.2} 
& \civ{97.3}{96.8}{97.5} 
& \civ{75.0}{74.8}{75.4} 
& \civ{24.9}{18.3}{25.2} 
& \civ{34.0}{32.0}{35.2} 
\\
\cit{~~Full (kNN)}
& \civ{91.4}{91.2}{91.6} 
& \civ{68.7}{68.4}{68.9} 
& \civ{72.2}{72.0}{72.3} 
& \civ{99.5}{99.5}{99.5} 
& \civ{95.4}{95.3}{95.4} 
& \civ{55.1}{55.1}{55.2} 
& \civ{75.3}{74.4}{77.4} 
& \civ{82.8}{82.5}{83.4} 
& \civ{94.8}{94.4}{95.1} 
& \civ{73.1}{72.1}{73.8} 
& \civ{83.4}{83.4}{83.5} 
& \civ{57.3}{55.3}{58.1} 
& \civ{54.4}{51.0}{57.7} 
& \civ{42.2}{41.8}{43.0} 
& \civ{60.6}{58.6}{62.2} 
& \civ{93.7}{88.9}{95.7} 
& \civ{67.0}{44.0}{71.3} 
& \civ{25.5}{25.3}{29.0} 
& \civ{41.5}{39.9}{42.2} 
\\
\cit{~~All Experts (kNN)}
& \civ{91.6}{91.4}{91.7} 
& \civ{68.5}{68.4}{68.6} 
& \civ{72.1}{72.0}{72.3} 
& \civ{99.5}{99.5}{99.5} 
& \civ{95.4}{95.3}{95.4} 
& \civ{55.1}{55.1}{55.2} 
& \civ{77.9}{71.8}{80.7} 
& \civ{82.9}{82.6}{83.2} 
& \civ{94.9}{94.7}{95.0} 
& \civ{73.7}{73.4}{73.9} 
& \civ{83.4}{83.3}{83.5} 
& \civ{61.0}{58.4}{61.8} 
& \civ{77.6}{74.2}{80.7} 
& \civ{45.6}{44.8}{46.4} 
& \civ{62.3}{60.0}{62.9} 
& \civ{87.6}{85.7}{90.6} 
& \civ{67.6}{66.8}{71.8} 
& \civ{25.3}{25.1}{25.6} 
& \civ{41.8}{40.9}{42.1} 
\\
\midrule
\emph{IN21k} & & & & & & & & & & & & & & & & & & & \\
\cit{~~Baseline}
& \civ{90.8}{90.7}{91.0} 
& \civ{72.5}{72.4}{72.6} 
& \civ{71.1}{71.0}{71.2} 
& \civ{98.5}{98.4}{98.5} 
& \civ{87.6}{87.4}{87.7} 
& \civ{48.6}{48.6}{48.7} 
& \civ{74.9}{72.6}{75.5} 
& \civ{84.3}{84.1}{84.5} 
& \civ{87.7}{73.4}{94.6} 
& \civ{73.2}{72.9}{73.8} 
& \civ{82.8}{82.2}{83.0} 
& \civ{52.2}{51.1}{53.4} 
& \civ{59.6}{58.1}{61.8} 
& \civ{42.1}{37.5}{43.2} 
& \civ{61.3}{60.0}{62.2} 
& \civ{95.4}{94.4}{96.0} 
& \civ{80.5}{78.7}{81.6} 
& \civ{30.6}{27.7}{30.7} 
& \civ{32.4}{29.7}{33.3} 
\\
\cit{~~Adapters (kNN)}
& \civ{89.9}{89.7}{90.9} 
& \civ{72.4}{72.3}{72.6} 
& \civ{71.2}{71.1}{71.3} 
& \civ{98.4}{98.4}{98.4} 
& \civ{89.4}{89.3}{89.6} 
& \civ{49.5}{49.4}{49.6} 
& \civ{75.8}{75.3}{76.2} 
& \civ{83.9}{83.1}{84.3} 
& \civ{94.6}{94.5}{94.6} 
& \civ{73.8}{73.2}{74.0} 
& \civ{81.8}{80.5}{82.0} 
& \civ{54.9}{53.5}{55.5} 
& \civ{64.0}{61.1}{68.4} 
& \civ{44.9}{44.2}{45.2} 
& \civ{61.3}{60.2}{61.9} 
& \civ{93.6}{91.4}{94.3} 
& \civ{78.6}{77.0}{79.5} 
& \civ{27.8}{27.7}{31.2} 
& \civ{34.9}{34.4}{35.6} 
\\
\cit{~~Full (kNN)}
& \civ{90.7}{90.3}{90.9} 
& \civ{72.5}{72.5}{72.5} 
& \civ{71.4}{71.4}{71.5} 
& \civ{98.6}{98.5}{98.6} 
& \civ{89.9}{89.4}{90.1} 
& \civ{49.7}{49.6}{49.7} 
& \civ{74.9}{74.5}{77.2} 
& \civ{83.8}{83.5}{84.2} 
& \civ{94.9}{94.8}{94.9} 
& \civ{73.6}{72.7}{74.0} 
& \civ{81.5}{81.5}{81.7} 
& \civ{58.2}{55.6}{59.4} 
& \civ{68.9}{65.8}{70.6} 
& \civ{45.1}{44.5}{45.7} 
& \civ{60.9}{59.5}{62.0} 
& \civ{95.3}{93.5}{96.2} 
& \civ{80.4}{79.7}{80.9} 
& \civ{31.1}{30.5}{31.8} 
& \civ{35.2}{34.7}{35.8} 
\\
\cit{~~All Experts (kNN)}
& \civ{90.8}{90.7}{90.9} 
& \civ{72.4}{72.2}{72.5} 
& \civ{71.4}{71.3}{71.4} 
& \civ{98.5}{98.4}{98.6} 
& \civ{89.6}{89.4}{90.1} 
& \civ{49.5}{49.5}{49.6} 
& \civ{76.0}{74.7}{77.5} 
& \civ{84.5}{84.0}{84.8} 
& \civ{94.8}{94.8}{94.9} 
& \civ{73.5}{73.2}{74.1} 
& \civ{81.4}{81.3}{81.5} 
& \civ{57.3}{55.2}{58.5} 
& \civ{68.3}{62.6}{72.1} 
& \civ{44.4}{44.3}{44.6} 
& \civ{61.4}{60.4}{62.0} 
& \civ{93.8}{92.1}{95.1} 
& \civ{80.2}{79.6}{80.7} 
& \civ{30.6}{30.1}{31.3} 
& \civ{34.3}{33.9}{35.4} 
\\
\midrule
\emph{JFT + IN21k} & & & & & & & & & & & & & & & & & & \\
\cit{~~All Experts (kNN)}
& \civ{90.7}{90.6}{90.8} 
& \civ{68.5}{68.4}{68.7} 
& \civ{71.4}{71.3}{71.5} 
& \civ{99.5}{99.5}{99.5} 
& \civ{95.4}{95.3}{95.4} 
& \civ{55.2}{55.1}{55.2} 
& \civ{80.6}{78.1}{81.5} 
& \civ{84.5}{84.3}{84.8} 
& \civ{94.9}{94.8}{94.9} 
& \civ{73.2}{72.1}{73.9} 
& \civ{83.5}{83.4}{83.6} 
& \civ{61.4}{60.6}{62.2} 
& \civ{78.1}{73.2}{81.8} 
& \civ{44.8}{44.0}{45.4} 
& \civ{62.5}{61.8}{63.0} 
& \civ{91.0}{88.1}{93.6} 
& \civ{66.9}{66.5}{67.9} 
& \civ{30.8}{27.7}{31.2} 
& \civ{40.9}{39.4}{41.7} 
\\
\bottomrule
\end{tabular}}

==> tables/vtab_literature.tex <==
\begin{tabular}{lrrrrr}
\toprule
& \textsc{Arch.} & \textsc{Nat.} & \textsc{Spec.} & \textsc{Str.} & \textsc{Avg.} \\
\midrule
ImageNet~\cite{zhai2019visual} & R50x1 & 72.6 & 82.2 & 51.1 & 65.6 \\
S4L-Rot~\cite{zhai2019visual} & R50x1 & 73.1 & 83.2 & 54.8 & 67.5 \\
VIVI-Co~\cite{tschannen2019selfsupervised} & R50x1 & 70.1 & 83.2 & \textbf{61.3} & 69.2 \\
BiT-I21k~\cite{kolesnikov2019large} & R50x1 & 72.6 & \textbf{86.4} & 54.4 & 67.6 \\
BiT-JFT~\cite{kolesnikov2019large} & R50x1 & 78.9 & \textbf{86.4} & 55.1 & 70.4 \\
All Experts-I21k (ours) & R50x1 & 78.3 & 83.6 & 58.8 & 71.2 \\
All Experts-JFT (ours) & R50x1 & \textbf{80.0} & 83.7 & 58.6 & \textbf{71.9} \\
\midrule
VIVI-Co-Big~\cite{tschannen2019selfsupervised} & R50x3 & 72.2 & 83.7 & 62.3 & 70.4 \\
BiT-JFT~\cite{kolesnikov2019large} & R50x3 & 82.7 & 88.3 & 56.2 & 72.7 \\
BiT-JFT~\cite{kolesnikov2019large} & R101x1 & 80.6 & 87.9 & 56.9 & 72.2 \\
BiT-JFT~\cite{kolesnikov2019large} & R152x4 & 86.0 & 87.0 & 62.2 & 76.2 \\
\bottomrule  
\end{tabular}  

==> tables/vtab_main_results.tex <==
\begin{tabular}{llllll}
\toprule
    & & \textsc{Natural} & \textsc{Specialized} & \textsc{Structured} & \textsc{All} \\
\midrule
\multirow{4}{*}{IN21k}
& Baseline 
& \cih{77.7}{77.4}{77.8} 
& \cih{82.0}{78.4}{83.9} 
& \cih{56.8}{55.9}{57.2}
& \cih{69.8}{68.8}{70.3} \\
& Adapters 
& \cih{78.1}{78.0}{78.3} 
& \cih{83.5}{83.1}{83.6}
& \cih{57.5}{56.8}{58.2}
& \cih{70.6}{70.3}{70.9} \\
& Full 
& \cih{78.3}{78.1}{78.6} 
& \cih{83.4}{83.2}{83.6} 
& \cih{59.4}{58.7}{59.8} 
& \cih{71.4}{71.1}{71.6} \\
& All Experts 
& \cih{78.3}{78.1}{78.6} 
& \cih{83.6}{83.4}{83.7} 
& \cih{58.8}{58.0}{59.4} 
& \cih{71.2}{70.8}{71.5} \\
\midrule
\multirow{4}{*}{JFT}
& Baseline 
& \cih{77.4}{77.3}{77.6} 
& \cih{81.6}{81.5}{82.0} 
& \cih{57.2}{52.8}{58.2} 
& \cih{69.8}{68.0}{70.2} \\
& Adapters 
& \cih{79.0}{78.6}{79.1} 
& \cih{81.3}{79.2}{82.5} 
& \cih{59.1}{58.3}{60.1} 
& \cih{71.1}{70.5}{71.6} \\
& Full 
& \cih{79.7}{79.5}{80.0} 
& \cih{83.6}{83.3}{83.8} 
& \cih{55.3}{52.2}{56.2} 
& \cih{70.2}{68.9}{70.6} \\
& All Experts
& \cih{80.0}{79.2}{80.4} 
& \cih{83.7}{83.6}{83.8} 
& \cih{58.6}{58.0}{59.4} 
& \cih{71.8}{71.3}{72.2} \\
\midrule
IN21k + JFT
& All Experts 
& \cih{\textbf{80.2}}{79.8}{80.3} 
& \cih{\textbf{84.0}}{83.7}{84.2} 
& \cih{\textbf{59.5}}{58.7}{60.1} 
& \cih{\textbf{72.3}}{71.9}{72.6} \\
\bottomrule  
\end{tabular}

==> tables/vtab_main_results_double_digit.tex <==
\begin{tabular}{llllll}
\toprule
    & & \textsc{Natural} & \textsc{Specialized} & \textsc{Structured} & \textsc{All} \\
\midrule
\multirow{4}{*}{IN21k}
& Baseline & \cih{77.71}{77.38}{77.81} & \cih{82.03}{78.43}{83.85} & \cih{56.77}{55.86}{57.16} & \cih{69.80}{68.84}{70.28} \\
& Adapters & \cih{78.10}{78.02}{78.26} & \cih{83.50}{83.08}{83.64} & \cih{57.51}{56.84}{58.24} & \cih{70.57}{70.27}{70.89} \\
& Full & \cih{78.25}{78.13}{78.58} & \cih{83.43}{83.20}{83.59} & \cih{59.39}{58.73}{59.77} & \cih{71.40}{71.12}{71.59} \\
& All Experts & \cih{78.31}{78.10}{78.55} & \cih{83.56}{83.41}{83.71} & \cih{58.79}{57.96}{59.42} & \cih{71.19}{70.83}{71.50} \\
\midrule
\multirow{4}{*}{JFT}
& Baseline & \cih{77.44}{77.33}{77.56} & \cih{81.60}{81.45}{81.98} & \cih{57.23}{52.76}{58.24} & \cih{69.81}{67.97}{70.24} \\
& Adapters & \cih{78.96}{78.59}{79.07} & \cih{81.34}{79.22}{82.48} & \cih{59.07}{58.30}{60.07} & \cih{71.09}{70.54}{71.56} \\
& Full & \cih{79.65}{79.51}{79.97} & \cih{83.55}{83.26}{83.80} & \cih{55.26}{52.19}{56.24} & \cih{70.20}{68.90}{70.63} \\
& All Experts & \cih{80.02}{79.17}{80.43} & \cih{83.72}{83.60}{83.82} & \cih{58.60}{57.95}{59.44} & \cih{71.78}{71.31}{72.19} \\
\midrule
IN21k + JFT
& All Experts 
& \cih{\textbf{80.19}}{79.79}{80.32} 
& \cih{\textbf{84.01}}{83.73}{84.21} 
& \cih{\textbf{59.54}}{58.71}{60.14} 
& \cih{\textbf{72.30}}{71.90}{72.56} \\
\bottomrule  
\end{tabular}
